Semantic Structure based Query Graph Prediction for Question Answering over Knowledge Graph

Building query graphs from natural language questions is an important step in complex question answering over knowledge graph (Complex KGQA). In general, a question can be correctly answered if its query graph is built correctly and the right answer is then retrieved by issuing the query graph against the KG. Therefore, this paper focuses on query graph generation from natural language questions. Existing approaches for query graph generation ignore the semantic structure of a question, resulting in a large number of noisy query graph candidates that undermine prediction accuracies. In this paper, we define six semantic structures from common questions in KGQA and develop a novel Structure-BERT to predict the semantic structure of a question. By doing so, we can first filter out noisy candidate query graphs, and then rank the remaining candidates with a BERT-based ranking model. Extensive experiments on two popular benchmarks MetaQA and WebQuestionsSP (WSP) demonstrate the effectiveness of our method as compared to state-of-the-arts.

==> last_ab_study_back.tex <==

\paragraph{The number of negative query graph:} Knowledge graph is a big database, for a question, it maps a plenty of negative query graph, but the high accuracy of ranking model is desired.
By statistics, we found the maximum of negative query graph for a question in WSP is more than 500 but less 600. We random 8 types negative query graph, their number are 1, 5, 10, 50, 100, 200, 300, 500. The results in Table \ref{ref:query graph analysis} show that the hits@1 value under 100 has the same result with the value under 300 (In this experiment, we fixed the added multi-head attention has one attention head, Pooling Layer is Mean Pooling). Otherwise, as shown in Table \ref{ref:query graph analysis}, when the number is 500, this ranking model has a lower performance than the model with 100. So the number of negative query graph has the impact for the hit@1 result.
%On the other hand, number 500 will lead model consume much more time.
%\textbf{Pooling operation} We evaluated the different pooling strategies in  TripleTransformer model, the results in Table \ref{ref:pooling} show that when we operate the ranking model, the Max pooling is slightly worse than the Mean pooling. 
\paragraph{Head number in added Transformer} We evaluate the performance of 3 types number of attention head in the added multi-attention layer, we found  the head number and hits@1 value are not positively linearly related. When the head number is 6, it just gets 70.63\%.

==> related_work_back.tex <==

\section{Related Work}
\subsection{Multi-hop Question Answering}
Current works on multi-hop question answering mainly focus on how to retrieve answers by calculating the relation paths step by step. In general, a right answer can be retrieved if the relation paths are identified correctly at each hop. \citet{Kun2019Enhancing} enhances the traditional Key-Value Memory Neural Networks (KV-MemNNs)~\cite{Miller2016Key} for multi-hop question answering. They design a query updating strategy to decompose the question and predict the relevant relation paths at each hop. TransferNet~\cite{shi2021transfernet} also calculates the relation path scores based on an updated question at each hop, but they leverage the attention mechanism to update question representations over multiple hops. More recently, \citet{cai2021deep} introduces the dual process theory to predict the relation paths at each hop. Although these methods achieve promising results, they suffer from error propagation when predicting the relation path step by step. To mitigate this issue, SSKGQA identifies the top-1 query graph by directly calculating the similarity scores between question and candidate query graphs (or similarly relation paths).

On the other hand, \citet{Sun2019PullNet,Sun2018Open} incorporate external corpus to enhance the performance of KGQA. First, they construct a subgraph for each question from KG and the Wikipedia documents. This subgraph stores the entities and text with a high probability to the topic entity and question. Afterwards, a Graph Neural Network (GNN)~\cite{Kipf2016Semi} is exploited to identify the final answer. A challenge of this method is that it is difficult to construct a subgraph around topic entity because we need to identify relevant entities from external corpus, and this process is error-prone. \citet{Apoorv2020Improving} predicts the answers by training a KG embedding model under a tuple of (topic entity, question, answer). However, complex questions with long relation paths can reduce the learnability of KG embedding significantly. Our SSKGQA does not need external corpus to improve prediction accuracies, and can solve complex multi-hop questions by a semantic structure based ranking model.

\subsection{Complex Questions with Constraints}

For questions with constraints, a sequence of works focus on how to reach the answers by generating query graphs. \citet{yih2015semantic} enumerates all possible entities and relation paths that connect with a topic entity to generate candidate query graphs, and uses a CNN-based ranking model to identify the query graph. Following a similar candidate query graph generation methods of \cite{yih2015semantic}, \citet{maheshwari2019learning} propose a novel query graph ranking method based on self-attention. \citet{qin2021improving} introduce a query graph generation method by using their proposed relation subgraphs. However, these methods largely ignore the noise when generating the candidate query graphs, which undermines the predictive performance during query graph ranking. To mitigate this issue, SSKGQA predicts the semantic structure of a question, which is then used to reduce the noise in candidate query graphs.



%constraints when generating query graphs at each step, and reduce the search space significantly.

%For questions with constraints, a sequence of works focus on how to reach the answers by generating query graphs. \citet{yih2015semantic} enumerates all possible entities and relation paths that connect with a topic entity to generate candidate query graphs, and uses a CNN-based ranking model to identify the query graph. \citet{maheshwari2019learning} follows the candidate query graph generation methods introduced in \citet{yih2015semantic} and propose a novel query graph ranking method based on self-attention. The most related work to ours is \citet{lan2020query} and \citet{chen2020formal}, \citet{lan2020query}  generates the  query graph by an iteration method at each step with considering the constraints. They perform constraints with predefined keyword. In contrast, in our proposed model, we make the query graph prediction without any predefined words.  \citet{chen2020formal} proposes a AQG generator which is used to predict the each vertex and edge in query graph step by step, this progress also can cause error cascade. Different from \citet{chen2020formal}, we try to summarize the semantic structure for the query graph, and predict the query graph for its whole structure.

\subsection{Query Graph Ranking}
Current research on KGQA mainly focuses on how to generate the candidate query graphs, and there are only a few works exploring how to rank the candidate query graphs. \citet{lan2020query} concatenates question and candidate query graph into a single sequence, and leverages BERT \cite{devlin2018bert} to process the whole sequence for ranking. However, \citet{reimers2019sentence} show that this strategy is inefficient as it can incur a massive computation due to the combinatorial nature of concatenation of question and candidate query graphs, leading to duplicated calculation. \citet{chen2020formal} explore GRUs to encode the question and query graph information, and utilize a hinge loss to learn a ranking model. However, GRUs can only learn a limited interaction among words in a sentence, while the global interactions among words has proven to be critical for text representation in various NLP applications~\cite{khan2020mmft}. To solve the aforementioned issues, SSKGQA exploits separated BERT models to process questions and query graphs, respectively, and reuses the extracted features to avoid duplicated calculation and leverages a triplet loss to train a BERT-based ranking model.
